The Parameterised Complexity of Integer Multicommodity Flow

The Integer Multicommodity Flow problem has been studied extensively in the literature. However, from a parameterised perspective, mostly special cases, such as the Disjoint Paths problem, have been considered. Therefore, we investigate the parameterised complexity of the general Integer Multicommodity Flow problem. We show that the decision version of this problem on directed graphs for a constant number of commodities, when the capacities are given in unary, is XNLP-complete with pathwidth as parameter and XALP-complete with treewidth as parameter. When the capacities are given in binary, the problem is NP-complete even for graphs of pathwidth at most 13. We give related results for undirected graphs. These results imply that the problem is unlikely to be fixed-parameter tractable by these parameters. In contrast, we show that the problem does become fixed-parameter tractable when weighted tree partition width (a variant of tree partition width for edge weighted graphs) is used as parameter.

==> old_gadgets.tex <==
% \subsubsection{Bifurcation}
% The second gadget is called a bifurcation gadget. The gadget is 
% not used in our proofs, but as later gadgets are generalisations
% of the construction, and the gadget may be useful for future
% proofs, we give it here.\jelle{Missing description of construction of gadget. Also, prime candidate to move to apppendix. Also, as there are no sources or sinks in this gadget, it is more dubious whether or not the choice gadget works entirely correct.}

% We assume that we must send $1$ flow through the gadget
% from $s_1$ to $t_1$ of commodity $1$ and that the top vertex can only receive flow of commodity 2.
% Now, all flow that the top vertex receives of commodity $2$ either has to be sent to the left branch
% or all has to be sent to the right branch: we cannot send a part of it to the left, and a part of
% it to the right branch.

% A similar bifurcation gadget can be used with the roles of the commodities reversed.

% Figure~\ref{figure:gadget2} shows how the gadget is constructed (right), and gives the schematic
% representation (left).

% \begin{lemma}
% Suppose that we have a flow where each arc departing from $s_1$ and each arc directed to $t_1$ is used with full capacity with commodity 1, and suppose $v$ only has incoming flow of commodity 2 of value $b\leq a$. Then either $v$ can send $b$ flow to $w$ and $0$ flow to $x$ through the gadget, or $0$ flow to $w$ and $b$ flow to $x$.
% \end{lemma}

% %We can also build a similar gadget with the roles of the commodities switched; these are drawn 90 degrees rotated.
% A bifurcation gadget has pathwidth $O(1)$, as each of the \chgad{a} gadgets has pathwidth $O(1)$. The size of the gadget is $O(a)$.

% \begin{figure}[htb]
%     \centering
%     \includegraphics[keepaspectratio,width=0.7\textwidth]{mcf-2}
%     \caption{Bifurcation gadget: At most $a_i$ flow is received in the gadget. All flow is either sent to the left or to the right. Note that the open circles represent \chgad{a} gadgets.}
%     \label{figure:gadget2}
% \end{figure}


